Quantum Gauge Field Theory in Cohesive Homotopy Type Theory

We implement in the formal language of homotopy type theory a new set of axioms called cohesion. Then we indicate how the resulting cohesive homotopy type theory naturally serves as a formal foundation for central concepts in quantum gauge field theory. This is a brief survey of work by the authors developed in detail elsewhere.

==> eptcsdata.tex <==
\providecommand{\firstpage}{109}
\providecommand{\publicationstatus}{R. Duncan and P. Panangaden (Eds.)\\
Quantum Physics and Logic 2012 (QPL2012)\\
EPTCS 158, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.158.8}{10.4204/EPTCS.158.8}}
\pdfoutput=1

